TimeFlows: Visualizing Process Chronologies from Vast Collections of Heterogeneous Information Objects

In many fact-finding investigations, notably parliamentary inquiries, process chronologies are created to reconstruct how a controversial policy or decision came into existence. Current approaches, like timelines, lack the expressiveness to represent the variety of relations in which historic events may link to the overall chronology. This obfuscates the nature of the interdependence among the events, and the texts from which they are distilled. Based on explorative interviews with expert analysts, we propose an extended, rich set of relationships. We describe how these can be visualized as TimeFlows. We provide an example of such a visualization by illustrating the Childcare Benefits Scandal -- an affair that deeply affected Dutch politics in recent years. This work extends the scope of existing process discovery research into the direction of unveiling non-repetitive processes from unstructured information objects.

==> sections/challenges.tex <==
In this article, we have several models by means of which we can understand temporal graphs, and discussed the relations among events and communication texts that experts value the most. Moreover, our proof of concept a glimpse of what a temporal graph would look like, if it adheres to the values and preferences of these experts. \par 

The recency of the articles that have appeared on temporal graphs models \cite{ansah2019} \cite{liu2020} \cite{noram2021}, and the lack of research on peoples' preferences regarding the structure, visualization and interactive elements comprising such temporal graphs, indicate that a substantial amount of work remains to be carried out. \par 

We therefore highlight a series of \emph{challenges} that help give direction to new research. We hope these challenges aid upcoming researchers, and provide a useful framework through which they can contextualize their own work and channel their efforts towards broadly applicable results effectively. 

\begin{enumerate}[noitemsep, start=1,label={(\bfseries C\arabic*)}]
\item Translate a sequence of words in each individual CT to a set of related \emph{concepts}. These concepts include topics, entities (actors, places, organizations), and other relevant classes of information. We call such a collection of related concepts a \emph{CT Ontology}. TODO: hier iets over Named Entity Recognition (NER) zeggen, als mogelijk toepasbare techniek? TODO: hier ook iets zeggen over probabilistische aard van de links tussen woorden en concepten? 
\item Embed these CT ontologies within a \emph{context}. TODO: hier its zeggen over Named Entity Linking (NML) als mogelijke techniek? 
\item Relate CTs by means of this context. There may be multiple types relations between CTs - including the topical, actoral and temporal relations described in this article.   
\item Identify \emph{events} within and among CTs by means of this context. TODO: hier nog wat zeggen over NLP-technieken, zoals sammenvatmethoden? 
\item Link these events to one another through different types of relations. 
\end{enumerate}

In addition to the five research challenges listed above, we wish to highlight a strand of research that spans all of them. This line of inquiry pertains to human-computer interaction. In this case, techniques from the field can be applied to allow for the presentation user-desired insights in the corpus of CTs, the context, the CT linkages, and the (links between the) events. Users should be able to continuously update their interests. This process is called \emph{keeping humans in the loop}. By means of this interactivity between the user and the software, the former ought to be able to generate appropriate visualizations of temporal graphs and their components. Moreover, analysts should have the capacity to iteratively adjust the level of granularity of events \cite{shahaf2013}, in order to optimally accommodate their research. 

==> sections/qualan.tex <==
\textbf{@ Jan Martijn} \emph{hier kun je het PDD in zetten en 'm kort beschrijven. Daarna zou er een sectie kunnen komen over de challenges van professionele tijdlijnmakers, maar ik vrees dat het niet gaat passen. Denk dat we een keuze moeten maken tussen professionele challenges in Sectie 3 en technische challenges in Sectie 4.} 

To gain an understanding of the qualitative data that that was gathered by conducting the interviews, we proceeded by means of a \emph{grounded theory approach} as follows. First, we recorded all of the interviews and saved them as audio files. Second, we transcribed the interviews. Next, we thoroughly read all of the texts that comprised the interview answers. While doing so, we underlined and circled the words and sentences that stood out most. Fourth, we made summaries of each individual interview. Fifth and finally, we analysed the summaries, looking for commonalities and particularities among the answers. We especially paid attention to the things the participants said about the different relationships between the texts they read in order to manufacture their timelines, and the events they extracted from them. \par

The interview transcripts and their summaries revealed both commonalities and differences in terms of the goals for, approach of, and document-event relations (implicitly) employed for the process of creating timelines. Let's start of with their respective goals or purposes. While the journalist made timelines to gain clarity of the events that were relevant to their topic of investigation, the parliamentary inquiry coordinators also had other goals in mind. Collecting the timelines from different ministries gave them insights as to how they comparatively experienced the same chain of events. Moreover, the junior council advisor mainly made the timelines and fact sheets to be able to assist the prime minister with the parliamentary inquiry hearings, and help them with recollecting the events and the role they played in them years ago. Thus, the timelines would aid the prime minister with answering questions from the hearing committee. Finally, the researchers of the ministry of Economic Affairs and Climate mainly made timelines to answer to the requests of the inquiry committee. Therefore, their timelines had to be written in a language that was as neutral as possible, and descriptions of events needed to be paraphrased in a manner that was as close to the descriptions in the original sources as possible. \par

\begin{figure}[H]
\centering
\fbox{\includegraphics[width=0.9\textwidth]{figures/procedure-tijdlijn-journalist.png} } 
\caption{}
\label{sketchprocessjournalist}
\end{figure}

The approaches partially overlapped with one another. Both the journalist and the ministry researchers started of by collecting relevant documents in a large file. Then, the researchers would proceed by adding more specific documents, based on the initial file collection. Subsequently, both the researchers and the journalist would create what the parliamentary coordinators called a \emph{chronology}. A chronology is a collection of dates and events. One could interpret it as a large proto-timeline, which hasn't been moulded into a timeline yet. Such a "true" timeline would afterwards be created based on subsections of the chronology. It usually pertains to a more specific theme or subject than the rough chronology. The researchers would sometimes also turn such a timeline into a fact sheet. Such a document is a more prosaic version of the timeline, written in the form of a short story. The goal of making such fact sheets is to make the chain of events more easily readable and memorable to humans. \par

\begin{figure}[H]
\centering
\fbox{\includegraphics[width=0.9\textwidth]{figures/procedure-tijdlijn-ezk.png} }
\caption{A rough sketch of the process of timeline-making for a group of researchers working at the Ministry of Economic Affairs in the Netherlands, formulated through the answers on interview questions} 
\label{sketchprocessezk}
\end{figure} 

The council advisor and the parliamentary started off differently. Both of them started off with chronologies. The coordinators would create such a chronology themselves. It sometimes would span hundreds of pages. Which events and dates are included in such a chronology, depends heavily on the intuition and experience of the researchers involved: "The human aspect in this procedure is very important... what is clearly involved is the human interpretation of the texts, and their judgement beforehand of what might be relevant."

The council advisor requested previously made chronologies - created by the ministries of Finance and Social Affairs - to aid them in their own work flows. With these "external" chronologies, the council advisor would subsequently create their own, internal chronology. Afterwards, this chronology would be cut into the twelve different timelines, corresponding to the respective topics communicated by the inquiry committee. These would also be made into different fact sheets, which would aid the prime minister during the hearings. \par

The coordinators aimed at comparing the different timelines they had claimed from the relevant ministries with one another. They would create their own timelines based on their (large) chronology, and compare it with the timelines claimed from the ministries. They would focus on the subjective aspects and outlooks of the different governing bodies they had requested timelines from. These comparisons would aid them in writing up the final report. \par
